Model-Free, Monotone Invariant and Computationally Efficient Feature Screening with Data-adaptive Threshold

Feature screening for ultrahigh-dimension, in general, proceeds with two essential steps. The first step is measuring and ranking the marginal dependence between response and covariates, and the second is determining the threshold. We develop a new screening procedure, called SIT-BY procedure, that possesses appealing statistical properties in both steps. By employing sliced independence estimates in the measuring and ranking stage, our proposed procedure requires no model assumptions, remains invariant to monotone transformation, and achieves almost linear computation complexity. Inspired by false discovery rate (FDR) control procedures, we offer a data-adaptive threshold benefit from the asymptotic normality of test statistics. Under moderate conditions, we demonstrate that our procedure can asymptotically control the FDR while maintaining the sure screening property. We investigate the finite sample performance of our proposed procedure via extensive simulations and an application to genome-wide dataset.

==> definition.tex <==
\usepackage{latexsym, amsbsy, amssymb,multirow, epsfig, amsmath}
\usepackage{hyperref}

%--------------------Initialize---------------------%
%\textheight= 9in  \textwidth = 6.5in \topmargin = -1.4cm
%\oddsidemargin = -0.15in \evensidemargin = 0in
\usepackage{graphicx,setspace,lscape,longtable}
\usepackage{epsfig,graphicx}
\usepackage{natbib}
\usepackage{subfigure}
\usepackage{floatrow}   
\usepackage{tikz}
\usepackage{comment}
%\usepackage{subcaption}
\usepackage{xcolor} 
\usepackage[framemethod=tikz]{mdframed}
\usepackage{amsmath,amsthm,amssymb,color}
\RequirePackage[mathlines, displaymath]{lineno}
\bibpunct{(}{)}{;}{a}{,}{,}

\setlength{\textwidth}{6.2in} \setlength{\textheight}{8.75in}
\setlength{\topmargin}{-0.25in} \setlength{\oddsidemargin}{0.25in}
\setlength{\evensidemargin}{0.25in}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}{Lemma}
%\newtheorem{prop}{Proposition}
\baselineskip = 7mm
\parskip = 2.5mm

%\usepackage{titlesec} % for redefine section
%\titleformat{\section} % command
%{\centering\large\bfseries} % shape
%{\thesection.} % sep
%{0.5em} % before
%{} % after
%
%
%\titleformat{\subsection}
%{\centering\it%
%}
%{\thesubsection.} %sep
%{0.5em}{}


%\newcommand{\csection}[1]
%    {
%\begin{center}
%        \stepcounter{section}
%        {\bf\large\arabic{section}. #1}
%    \end{center}
%    \vspace{-0.15 cm}
%}

%\newcommand{\csubsection}[1]{
%\vspace{-0.25 cm}
%\begin{center}
%\stepcounter{subsection}
%{\it\arabic{section}.\arabic{subsection}. #1}
%\end{center}
%\vspace{-0.25 cm}
%}
\newcommand{\scsection}[1]
    {\begin{center}
        {\bf\large #1}
    \end{center}
    \vspace{-0.15 cm}
}

%% To create ref
\newcounter{csection}
\newcommand{\csection}[1]
    {
        \refstepcounter{csection}
\begin{center}
        {\bf\large\arabic{csection}. #1}
    \end{center}
    \vspace{-0.15 cm}
}

\newcounter{csubsection}[csection]
\renewcommand{\thecsubsection}{\thecsection.\arabic{csubsection}}

\newcommand{\csubsection}[1]{
\refstepcounter{csubsection}%
\vspace{-0.25 cm}
\begin{center}
{\it\arabic{csection}.\arabic{csubsection}. #1}
\end{center}
\vspace{-0.25 cm}
}

\newcommand{\scsubsection}[1]{
\vspace{-0.25 cm}
\begin{center}
\stepcounter{subsection}
{\it #1}
\end{center}
\vspace{-0.25 cm}
}

\def\beqr{\begin{eqnarray}}
\def\eeqr{\end{eqnarray}}
\def\beqrs{\begin{eqnarray*}}
\def\eeqrs{\end{eqnarray*}}
\def\bep{\begin{prop}}
\def\eep{\end{prop}}

\def\mR{\mathbb{R}}
\def\calA{\mathcal{A}}
\def\calB{\mathcal{B}}
\def\calC{\mathcal{C}}
\def\calD{\mathcal{D}}
\def\calF{\mathcal{F}}
\def\calH{\mathcal{H}}
\def\calI{\mathcal{I}}
\def\calS{\mathcal{S}}
\def\calP{\mathcal{P}}
\def\calM{\mathcal{M}}
\def\calN{\mathcal{N}}
\def\calU{\mathcal{U}}
\def\calT{\mathcal{T}}
\def\calH{\mathcal{H}}
\def\calR{\mathcal{R}}
\def\calX{\mathcal{X}}
\def\calY{\mathcal{Y}}
\def\calZ{\mathcal{Z}}

%\newtheorem{Theorem}{Theorem}[section]
%\newtheorem{Corollary}{Theorem}[section]
%\newtheorem{Lemma}[Theorem]{Lemma}




\def\bias{\mbox{bias}}
\def\pr{\mbox{pr}}
\def\var{\mbox{var}}
\def\cov{\mbox{cov}}
\def\cor{\mbox{cor}}
\def\MSE{\mbox{MSE}}
\def\arcos{\mbox{arcos}}

\textheight= 9in
\textwidth = 6.1in
\evensidemargin = 0in
\renewcommand{\thefootnote}{\fnsymbol{footnote}}


%\numberwithin{equation}{section}
\numberwithin{equation}{csection}
\renewcommand{\baselinestretch}{1.75}


%\bibliographystyle{cheng}
%\renewcommand\refname{REFERENCE}
\bibliographystyle{refstyle1}
\renewcommand\refname{REFERENCE}


%-------------Li-Ping's Definition-----------------------%
\def\hDash{\bot\!\!\!\bot}
\def\wh{\widehat}
\def\wt{\widetilde}
\def\ba{\mbox{\boldmath$\alpha$}}
\def\bb{\mbox{\boldmath$\beta$}}
\def\bg{\mbox{\boldmath$\gamma$}}
\def\ha{\mbox{$\widehat\ba$}}
\def\hb{\mbox{$\widehat\bb$}}
\def\hg{\mbox{$\widehat\bg$}}
\def\hDash{\bot\!\!\!\bot}


\def\a{{\bf a}}
\def\b{{\bf b}}
\def\A{{\bf A}}
\def\B{{\bf B}}
\def\C{{\bf C}}
\def\G{{\bf G}}
\def\X{{\bf X}}
\def\x{{\bf x}}
\def\Y{{\bf Y}}
\def\y{{\bf y}}
\def\Z{{\bf Z}}
\def\z{{\bf z}}
\def\u{{\bf u}}
\def\s{{\bf s}}
\def\t{{\bf t}}
\def\h{{\bf h}}
\def\k{{\bf k}}
\def\l{{\bf l}}
\def\c{{\bf c}}
\def\d{{\bf d}}
\def\w{{\bf w}}
\def\g{{\bf g}}
\def\I{{\bf I}}
\def\R{{\bf R}}
 \def\vo{{\bf 1}}
\def\vz{{\bf 0}}

\def\balpha{{\bm \alpha}}
\def\bbeta{{\bm \beta}}
\def\bzeta{{\bm \zeta}}
\def\betaa{{\bm \eta}}
\def\bome{{\bm \omega}}
\def\bpi{{\bm \pi}}

\newcommand{\trans}{^{\mbox{\tiny{T}}}}
\def\defby{\stackrel{\mbox{\textrm{\tiny def}}}{=}}

\newcommand{\beps}{\mbox{\boldmath $\varepsilon$}}
\newcommand{\bSig}{\mbox{\boldmath $\Sigma$}}
\newcommand{\hSig}{\mbox{$\widehat{\bSig}$}}
\newcommand{\bLam}{\mbox{\boldmath $\Lambda$}}
\newcommand{\hLam}{\mbox{$\widehat{\bLam}$}}
\newcommand{\bOmega}{\mbox{\boldmath $\Omega$}}
\newcommand{\bI}{\mbox{\boldmath $I$}}
\newcommand{\bGam}{\mbox{\boldmath $\Gamma$}}

\newtheorem{defi}{\sc Definition}[section]
\newtheorem{theo}{\bf Theorem}
\newtheorem{lemm}{\sc Lemma}
\newtheorem{prop}{\sc Proposition}
\newtheorem{coll}{\sc Corollary}[theo]
\newtheorem{rema}{\bf Remark}
\newtheorem{exam}{\bf Example}



\def\diamondplus{\mathrel{%
		\ooalign{\raise.29ex\hbox{$\scriptscriptstyle+$}\cr\hss$\diamond$\hss}}}

%--------------------------------------------------------------%


\headsep 6pt
\topmargin 0in
\textheight 8.5in
\evensidemargin 0.5in
\oddsidemargin 0.5in
\textwidth 6in
\footskip 18pt


\newtheorem*{non-lemma}{\sc Lemma}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}


\newcommand{\skipline}{\vspace{12pt}}
\newcommand{\Rcor}{{\rm{Rcor}}}
\newcommand{\Scor}{{\rm{Scor}}}
\newcommand{\Dcov}{{\rm{Dcov}}}
\newcommand{\GDcov}{{\rm{GDcov}}}
\newcommand{\Pcov}{{\rm{Pcov}}}
\newcommand{\Acov}{{\rm{Acov}}}
\newcommand{\DC}{{{\rm DC}}}
\newcommand{\PC}{{{\rm PC}}}
\newcommand{\AC}{{{\rm AC}}}
\newcommand{\BPC}{{{\rm BPCor}}}
\newcommand{\PCPR}{{{\rm PCPR}}}
\newcommand{\HSIC}{{{\rm HSIC}}}

\newcommand{\D}{\mbox{D}}
\newcommand{\E}{\mbox{E}}
\newcommand{\F}{\mbox{F}}
\newcommand{\NLS}{\mbox{NLS}}
\newcommand{\GPLSIM}{\mbox{GPLSIM}}
\newcommand{\Known}{\mbox{Known}}
\newcommand{\PS}{\mbox{PS}}
\newcommand{\PR}{\mbox{PR}}
\newcommand{\LS}{\mbox{LS}}
\newcommand{\LSR}{\mbox{LSR}}
\newcommand{\PPR}{\mbox{PPR}}
\newcommand{\SIR}{\mbox{SIR}}
\newcommand{\pHd}{\mbox{pHd}}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\vech}{\mbox{vech}}
\newcommand{\mvz}{\mbox{${\bf z}$}}
\newcommand{\Hessian}{\mbox{${\bf H}$}}

\newcommand{\ang}{{\rm{ang}}}


\newcommand{\yvec}{\mbox{\boldmath $y$}}

\newcommand{\Zvec}{\mbox{\boldmath $Z$}}
\newcommand{\avec}{\mbox{\boldmath $a$}}
\newcommand{\bvec}{\mbox{\boldmath $b$}}
\newcommand{\mvec}{\mbox{\boldmath $m$}}
\newcommand{\svec}{\mbox{\boldmath $s$}}
\newcommand{\tvec}{\mbox{\boldmath $t$}}
\newcommand{\uvec}{\mbox{\boldmath $u$}}
\newcommand{\wvec}{\mbox{\boldmath $w$}}
\newcommand{\gammavec}{\mbox{\boldmath $\gamma$}}
\newcommand{\epsvec}{\mbox{\boldmath $\epsilon$}}
\newcommand{\zetavec}{\mbox{\boldmath $\zeta$}}
\newcommand{\etavec}{\mbox{\boldmath $\eta$}}
\newcommand{\thetavec}{\mbox{\boldmath $\theta$}}
\newcommand{\chivec}{\mbox{\boldmath $\chi$}}
\newcommand{\Covmat}{\mbox{\boldmath $\Sigma$}}
\newcommand{\Bmat}{\mbox{${\bf B}$}}

% \newcommand{\norm}{\|} % commented by ccy
\usepackage{latexsym}
\usepackage{epsfig}
\usepackage{bm}

\usepackage{threeparttable}
\usepackage{booktabs}
%\usepackage{siunitx,booktabs} % table row space
%\sisetup{separate-uncertainty}
%\renewcommand{\baselinestretch}{1.75}
%
%\newcommand{\csection}[1]
%{\begin{center}
%		\stepcounter{section}
%		{\bf\large\arabic{section}. #1}
%	\end{center}
%	\vspace{-0.15 cm}}
%\newcommand{\scsection}[1]
%{\begin{center}
%		{\bf\large #1}
%	\end{center}
%	\vspace{-0.15 cm}}
%\newcommand{\csubsection}[1]{
%	\vspace{-0.25 cm}
%	\begin{center}
%		\stepcounter{subsection}
%		{\it\arabic{section}.\arabic{subsection}. #1}
%	\end{center}
%	\vspace{-0.25 cm}}
%\newcommand{\scsubsection}[1]{
%	\vspace{-0.25 cm}
%	\begin{center}
%		\stepcounter{subsection}
%		{\it #1}
%	\end{center}
%	\vspace{-0.25 cm}}
%
%
%
%
%%\usepackage{xr}
%%\externaldocument{其他文件名称，可以引用其他文件中出现的标号} % 例如，
%\usepackage{xr}
%\externaldocument{chap1}
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					可能需要使用特殊的一些包    			    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\RequirePackage[mathlines, displaymath]{lineno}
%\usepackage{natbib}
%\usepackage{latexsym, amsbsy, amssymb,multirow, epsfig, amsmath}
%\usepackage[left=30mm,right=28mm,top=2cm,bottom=2cm]{geometry}
%%\usepackage{amssymb,amsthm,amsmath,mathrsfs,bm,color}
%%\setlength{\textwidth}{6.2in} \setlength{\textheight}{8.75in}
%%\setlength{\topmargin}{-0.25in} \setlength{\oddsidemargin}{0.25in}
%%\setlength{\evensidemargin}{0.25in}
%%\usepackage{hyperref}
%%\baselineskip = 7mm
%%\parskip = 2.5mm
%%
%%\textheight= 9in
%%\textwidth = 6.1in
%%\evensidemargin = 0in
%%
%
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					可能需要使用特殊的命令行    			    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\beqr{\begin{eqnarray}}
%\def\eeqr{\end{eqnarray}}
%\def\beqrs{\begin{eqnarray*}}
%\def\eeqrs{\end{eqnarray*}}
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出比较常用的定理环境定义  	   	   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\newtheorem{theo}{\bf Theorem}
%\bibliographystyle{refstyle}
%\renewcommand\refname{REFERENCE}
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出比较常用的特殊算子定义  		   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\pr{\mbox{pr}}
%\def\cov{\mbox{cov}}
%\def\var{\mbox{var}}
%\def\sign{\mbox{sign}}
%\def\sp{\textrm{span}}
%\def\vecl{\textrm{vecl}}
%
%
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出比较常用的特殊符号定义  		   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\mR{\mathbb{R}}
%\def\calA{\mathcal{A}}
%\def\calB{\mathcal{B}}
%\def\calC{\mathcal{C}}
%\def\calD{\mathcal{D}}
%\def\calI{\mathcal{I}}
%\def\calN{\mathcal{N}}
%\def\calS{\mathcal{S}}
%\def\calX{\mathcal{X}}
%\def\calY{\mathcal{Y}}
%\def\calZ{\mathcal{Z}}
%
%
%\def\a{{\bf a}}
%\def\b{{\bf b}}
%\def\c{{\bf c}}
%\def\d{{\bf d}}
%\def\u{{\bf u}}
%\def\v{{\bf v}}
%\def\w{{\bf w}}
%\def\x{{\bf x}}
%\def\y{{\bf y}}
%\def\z{{\bf z}}
%
%\def\A{{\bf A}}
%\def\B{{\bf B}}
%\def\C{{\bf C}}
%\def\D{{\bf D}}
%\def\I{{\bf I}}
%\def\X{{\bf X}}
%\def\Y{{\bf Y}}
%\def\Z{{\bf Z}}
%
%
%\def\ba{\mbox{\boldmath$\alpha$}}
%\def\bb{\mbox{\boldmath$\beta$}}
%\def\bSig{\mbox{\boldmath$\Sigma$}}
%
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%%                      																								  %
%%                      					给出其他一些的特殊算子定义  		   	    			 %
%%                      																								  %
%% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
%\def\defby{\stackrel{\mbox{\textrm{\tiny def}}}{=}}
%\newcommand{\trans}{^{\mbox{\tiny{T}}}}
%\def\hDash{\bot\!\!\!\bot}
%\def\wh{\widehat}
%\def\wt{\widetilde}



% --------------- Added by ccy ----------------------- %
% norm & abs
\newcommand{\norm}[1]{\Vert#1\Vert}
\newcommand{\Norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\inner}[2]{\langle #1, #2 \rangle}
\newcommand{\Inner}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\abs}[1]{\vert#1\vert}
\newcommand{\Abs}[1]{\left\vert#1\right\vert}


\usepackage{enumitem} % redefine enumerate


\usepackage[colorinlistoftodos]{todonotes} % for todo

\usepackage{tikz}

\usepackage{amssymb}


\usepackage{threeparttable}
\usepackage{multirow}

% for caption below table, cf. https://latex.org/forum/viewtopic.php?t=5572.
\usepackage{caption}


\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}

\DeclareMathOperator\supp{supp}


% --------------- Added by dls ----------------------- %
\newcommand{\linsuiq}[1]{{\bf\textcolor{red}{[Linsui(Q): #1]}}}
\newcommand{\FDR}{\mathrm{FDR}}
\newcommand{\FDP}{\mathrm{FDP}}

\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}
\newcommand{\rNum}[1]{\lowercase\expandafter{\romannumeral #1\relax}}
\usepackage{soul}
% Create subtheorems

  
\newcounter{subtheo}[theo]
\renewcommand{\thesubtheo}{(\textit{\alph{subtheo}})}
\makeatletter
\renewcommand{\p@subtheo}{\thetheo}% Counter prefix.
\makeatother
\newcommand{\subtheo}{% Just like \item in a list, but for an asu
  \refstepcounter{subtheo}%
  \thesubtheo~\ignorespaces}


\makeatletter
\newcommand{\mylabel}[2]{#2\def\@currentlabel{#2}\label{#1}}
\makeatother
